How Likely Do LLMs with CoT Mimic Human Reasoning?

Chain-of-thought emerges as a promising technique for eliciting reasoning capabilities from Large Language Models (LLMs). However, it does not always improve task performance or accurately represent reasoning processes, leaving unresolved questions about its usage. In this paper, we diagnose the underlying mechanism by comparing the reasoning process of LLMs with humans, using causal analysis to understand the relationships between the problem instruction, reasoning, and the answer in LLMs. Our empirical study reveals that LLMs often deviate from the ideal causal chain, resulting in spurious correlations and potential consistency errors (inconsistent reasoning and answers). We also examine various factors influencing the causal structure, finding that in-context learning with examples strengthens it, while post-training techniques like supervised fine-tuning and reinforcement learning on human feedback weaken it. To our surprise, the causal structure cannot be strengthened by enlarging the model size only, urging research on new techniques. We hope that this preliminary study will shed light on understanding and improving the reasoning process in LLM.

==> figures/accuracy_direct_vs_cot.tex <==
\begin{figure*}[h]
    \centering
    \setlength{\abovecaptionskip}{6pt}    
    \includegraphics[width=1.0\linewidth]{sources/accuracy_direct_vs_cot.pdf}   
    \caption{LLMs with CoT exhibit \emph{inconsistent effects}, where the CoT shows inferior performance to Direct in the tasks on the left but superior performance in the tasks on the right in a zero-shot setting. We use a line chart instead of a bar chart to illustrate the trends from small to large models. (See Table \ref{tab:direct_vs_cot.result} in Appendix \ref{app:detailed_results} for the detailed results.)}
    \label{fig:accuracy_direct_vs_cot}
\end{figure*}

==> figures/cotnshot_bias.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.95\linewidth]{sources/cotnshot_bias.pdf}   
    \caption{Impact of ICL (n-shot) on the accuracy and the treatment effect of random bias, where the demonstration examples enhance the results but also introduce variance, and the treatment effect is especially influenced by the number of examples. The rise in both accuracy and variance indicates a trend that aligns with prior research on demonstrations \cite{zhang2023understanding}.}
    \label{fig:cotnshot_bias}
\end{figure*}

==> figures/intro.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{sources/intro.pdf}   
    \caption{There is a discrepancy between the expected behavior and the real behavior of CoT, but the root cause remains unclear.}
    \label{fig:intro}
\end{figure}

==> figures/intro2.tex <==
\begin{figure}[h!]
    \begin{subfigure}[b]{0.6\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth,trim={0 0mm 0 0mm},clip]{sources/intro1.pdf}   
        \caption{CoT is expected to causally determine the answer.}
        \label{fig:intro-causal}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth,trim={0 0mm 0 0mm},clip]{sources/intro2.pdf}   
        \caption{However, CoT and Answer do not always align in practice. }
        \label{fig:intro-gap}
    \end{subfigure}
    \caption{There is a discrepancy between the expected behavior and the real behavior of CoT, but the root cause remains unclear.}
\end{figure}



==> figures/superficial_cot.tex <==
\begin{figure*}[h!]
% \begin{wrapfigure*}{r}{0.5\textwidth}
\centering
\scriptsize
\resizebox{0.96\textwidth}{!}{
\begin{AIbox}{Superficial features in CoT}
{
\begin{tcolorbox}[colback=blue!20, bottom=1pt, top=1pt, left=1pt, right=1pt]
{\bf Question:} Your goal is to reason step by step to solve the logical reasoning problem. Given a context and a question, explain your reasoning process and give the answer with the format "\textbackslash nThe correct option is: A/B/C".\newline
\# Context:\newline
Bob is not round. Charlie is furry. Charlie is nice. Charlie is smart. Erin is red. Fiona is furry. Fiona is young. All red people are not round. Red people are not blue. All young people are furry. If Erin is red and Erin is not round then Erin is nice. If someone is round and nice then they are not young. All smart people are young. Nice people are smart."\newline
\# Question:
Based on the above information, is the following statement true, false, or unknown? Erin is furry.\newline
\# Options:\newline
A) True
B) False
C) Unknown\newline
\# Instruction:\newline
\#\# Reasoning:
\end{tcolorbox}
}
{
\begin{tcolorbox}[colback=yellow!20, bottom=1pt, top=1pt, left=1pt, right=1pt]
{\bf Answer:} First, let's analyze the given information:\newline
- Erin is red.\newline
- All red people are not round.\newline
- If Erin is red and Erin is not round then Erin is nice.\newline
- All young people are furry.\newline
- All smart people are young.\newline
- Nice people are smart.\newline
From the given information, we can conclude that Erin is not round, and she is nice. Since all red people are not round and Erin is red, it follows that Erin is not round. Additionally, if Erin is red and not round, then she is nice. Therefore, Erin is nice.\newline
Now, based on the information that \red{all young people are furry, and Erin is red, we can conclude that Erin is furry}.\newline
Therefore, the statement ``Erin is furry'' is true.\newline
The correct option is: A) True
\end{tcolorbox}
}

\end{AIbox}
}

\caption{An example of an erroneous CoT that relies on superficial features to deduce the right conclusion. The text in \red{red} underscores the flawed logic, omitting two essential preliminary steps: ``\emph{Nice people are smart. So, Erin is smart.}'' and ``\emph{All smart people are young. So, Erin is young.}''}
\label{fig:Superficial features in CoT}
\end{figure*}

==> tables/ProofWriter_Acc_on_Golden_CoT.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lcc}
\hline
Setting & gpt-3.5-turbo & gpt-3.5-turbo-instruct \\ 
\hline
Disrupt CoT & & \\ \hline
\quad w/ golden CoT & 0.73 & 0.75 \\ 
\quad\quad w/ golden CoT Role Chef & 0.80 & 0.61 \\
\quad\quad w/ golden CoT Role Detective & 0.72 & 0.65 \\ \hline
\quad w/ wrong CoT & 0.37 & 0.39 \\
\hline
\end{tabular}
\caption{Performance of ProofWriter with ChatGPT with golden CoT in Various Role Prompts}
\label{tab:chatgpt_roles}
\end{table*}


==> tables/ProofWriter_Acc_on_No_Context.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lcc}
\hline
Disrupt Context & gpt-3.5-turbo & gpt-3.5-turbo-instruct \\ \hline
\quad w/o context and w/ golden CoT & 0.54 & 0.74 \\ \hline
\quad w/o context and w/ golden Role Chef & 0.39 & 0.61 \\ \hline
\quad w/o context and w/ golden Role Detective & 0.42 & 0.66 
\end{tabular}
\caption{Performance of ProofWriter with ChatGPT with golden CoT in Various Role Prompts}
\label{tab:chatgpt_roles}
\end{table*}


==> tables/ProofWriter_Acc_on_Role.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lcc}
\hline
Setting & gpt-3.5-turbo & gpt-3.5-turbo-instruct \\
\hline
Direct Answer & 0.32 & 0.43 \\
CoT Baseline & 0.54 & 0.51 \\
\hline
Role Enhanced & & \\
\quad Mathematician & 0.55 & 0.44 \\
\quad Detective & 0.55 & 0.46 \\
\quad MathTeacher & 0.55 & 0.48 \\
\quad Philosopher & 0.54 & 0.47 \\
\quad EnglishTeacher & 0.53 & 0.46 \\
\quad PhysicalTeacher & 0.53 & 0.47 \\
\quad PrimarySchoolStudent & 0.52 & 0.49 \\
\quad Chef & 0.50 & 0.44 \\
\quad Scientist & 0.49 & 0.44 \\
\quad Judge & 0.47 & 0.45 \\
\hline
\end{tabular}
\caption{Performance of ProofWriter with ChatGPT in Various Role Prompts}
\label{tab:chatgpt_roles}
\end{table*}


==> tables/ProofWriter_w_bias.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lcccccccc}
\hline
\bf Setting & \multicolumn{2}{c}{\bf ProofWriter} & \multicolumn{2}{c}{\bf FOLIO} & \multicolumn{2}{c}{\bf LOGIQA} & \multicolumn{2}{c}{\bf GSM8K}\\ 
\hline
Add bias option & strong & weak & strong & weak & strong & weak & strong & weak \\ \hline
\quad CoT & 0.518 & 0.518 & 0.574 & 0.574 & 0.465 & 0.465\\
\quad\quad CoT w/ wrong option bias  & 0.392 & 0.403 & 0.363 & 0.451 & 0.192 & 0.253 \\
\hline
\quad w/ default CoT & 0.52 & 0.52 & 0.588 & 0.588 & 0.478 & 0.478\\ 
\quad\quad w/ default CoT + wrong option bias & 0.502 & 0.518 & 0.564 & 0.574 & 0.445 & 0.457 \\
\hline
\quad w/ golden CoT & 0.782 & 0.782 \\ 
\quad\quad w/ golden CoT + wrong option bias & 0.645 & 0.8 \\ 
\hline
\quad w/ random CoT & 0.352 & 0.352 \\ 
\quad\quad w/ random CoT + right option bias & 0.382 & 0.31\\ 
\hline
\end{tabular}
\caption{Performance of ProofWriter with bias option.}
\label{tab:chatgpt_roles}
\end{table*}


==> tables/chat_vs_instruct.result.tex <==
\begin{table*}[h]
    \centering\small
    \begin{tabular}{lcccccc}
        \hline
        \multirow{2}{*}{\bf Intervention} & \multicolumn{3}{c}{\bf Instruct} & \multicolumn{3}{c}{\bf 2-Shot}  \\ 
        & {\bf Addition} & {\bf Product} & {\bf ProofWriter} & {\bf Addition} & {\bf Product} & {\bf ProofWriter} \\
        \hline
        {\bf CoT} &  &  \\
        \multicolumn{7}{c}{\bf Test: If CoT causes Answer given constant Instruction?} \\
        Controlled (w/ default setting) & &  \\
        \quad Treated (w/ golden CoT) & &    \\ 
        \quad Treated (w/ random CoT) & &   \\
        CoT $\rightarrow$ Answer & &  \\
        \multicolumn{7}{c}{\bf Test: If Instruction causes Answer given constant CoT?} \\
        Controlled (w/ default setting) & &  \\
        \quad Treated (w/ random role) & &  \\
        \quad Treated (w/ random bias) & &   \\
        Controlled (w/ golden CoT) & &  \\
        \quad Treated (w/ random bias) & &  \\       
        Instruction $\rightarrow$ Answer & &  \\
        \hline
    \end{tabular}
    \caption{Chat vs Instruct. }
    \label{tab:chat_vs_instruct.result}
\end{table*}


==> tables/cot_intervention.implied_scm_mistral.tex <==
\begin{table*}[h]
    \centering\scriptsize
    % \setlength{\abovecaptionskip}{6pt}    
    % \setlength{\belowcaptionskip}{-9pt} 
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{l|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c|c}
        \hline
        \multirow{2}{*}{\bf Model} & \multicolumn{7}{c}{\bf CoT $\overset{?}{\longrightarrow}$ Answer ($\uparrow$)}  & \multicolumn{7}{c}{\bf Instruction $\overset{?}{\longrightarrow}$ Answer ($\downarrow$)} & \bf Avg. \\ 
        & \bf Add. & \bf Mul. & \bf GSM. & \bf Pro. & \bf FOL. & \bf LQA. & \bf Avg. $|\text{ATE}|$ & \bf Add. & \bf Mul. & \bf GSM. & \bf Pro. & \bf FOL. & \bf LQA. & \bf Avg. $|\text{ATE}|$ & \bf Accuracy \\
        \hline
        Base & F & T & T & T & F & T & \bf 0.204 & F & T & T & T & T & F & 0.111 & \bf 0.313 \\
        SFT & F & T & T & T & F & \it \red{F} & 0.179 & \it \red{T} & T & T & T & T & \it \red{T} & 0.156 & 0.300  \\
        DPO & F & T & T & T & F & \red{\it T} & 0.138 & T & \red{\it F} & T & T & \it \red{F} & T & \bf 0.066 & 0.275 \\
        \hline
    \end{tabular}
    \caption{The impact of SFT/DPO on causal relationships based on \emph{Mistral-7B}, where SFT primarily enhances the causal connection between the instruction and answer, and DPO diminishes this relationship. The detailed outcomes of the Base, SFT, and DPO models can be found in Table \ref{tab:cot_intervention.result_mistral_base}, \ref{tab:cot_intervention.result_mistral_sft}, and \ref{tab:cot_intervention.result_mistral_dpo} in Appendix \ref{app:detailed_results}, respectively.}
    \label{tab:cot_intervention.implied_scm_mistral}
\end{table*}


==> tables/cot_intervention.implied_scm_nshot.tex <==
\begin{table*}[h]
    \centering\scriptsize
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{l|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c|c}
        \hline
        \multirow{2}{*}{\bf ICL} & \multicolumn{7}{c}{\bf CoT $\overset{?}{\longrightarrow}$ Answer} & \multicolumn{7}{c}{\bf Instruction $\overset{?}{\longrightarrow}$ Answer} & \bf Avg.\\ 
        & \bf Add. & \bf Mul. & \bf GSM. & \bf Pro. & \bf FOL. & \bf LQA. & \bf Avg. $|\text{ATE}|$ & \bf Add. & \bf Mul. & \bf GSM. & \bf Pro. & \bf FOL. & \bf LQA. & \bf Avg. $|\text{ATE}|$ & \bf Accuracy \\
        \hline
        0-shot & F & T & T & T & T & T & 0.208 & T & T & F & T & F & T & 0.122 & 0.572 \\
        2-shot & \it \red{T} & T & T & T & T & T & 0.251 & T & T & F & T & \it \red{T} & \it \red{F} & 0.059 & \bf 0.598 \\
        4-shot & F & T & T & T & T & \it \red{F} & 0.059 & T & T & F & T & \it \red{T} & \it \red{F} & 0.049 & 0.580 \\
        8-shot & \it \red{T} & T & T & T & T & T & 0.229 & T & T & F & T & \it \red{T} & \it \red{F} & 0.065 & 0.592 \\
        \hline
    \end{tabular}
    \caption{The impact of ICL on causal relationships tested in \emph{GPT-3.5-Turbo}, where ICL examples primarily alter the intensity of the causal link between the instruction and answer. The detailed outcomes of the 0/2/4/8-shot can be found in Table \ref{tab:cot_intervention.result_chatgpt} and Table \ref{tab:cot_intervention.result_chatgpt_2shot}, \ref{tab:cot_intervention.result_chatgpt_4shot},  \ref{tab:cot_intervention.result_chatgpt_8shot} in Appendix \ref{app:detailed_results}, respectively.}
    \label{tab:cot_intervention.implied_scm_nshot}
\end{table*}


==> tables/cot_intervention.result_nshot.tex <==
\begin{table*}[h!]
    \caption{Interventions to identify the causes of the answer in \emph{GPT-3.5-Turbo with n-shot}, where the ICL examples have a significant impact on the Addition task, altering its implied SCM types.}
    \centering\scriptsize
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{@{}l|cccc|cccc@{}}
        \hline
        \multirow{2}{*}{\bf Intervention} & \multicolumn{4}{c}{\bf Addition} & \multicolumn{4}{c}{\bf Multiplication}  \\ 
         & 0-Shot & 4-Shot & 8-Shot & 16-Shot & 0-Shot & 4-Shot & 8-Shot & 16-Shot \\
        \hline
        CoT & 0.674 & 0.380 & 0.456 & 0.468 & 0.450 & 0.670 & 0.636 & 0.648 \\
        \hline
        \multicolumn{7}{c}{\bf Test: If CoT causes Answer given constant Instruction?} \\
        \grayline
        Controlled (w/ default setting) & 0.782 & 0.354 & 0.414 & 0.410 & 0.454 & 0.672 & 0.650 & 0.672 \\
        \quad\it Treated (w/ golden CoT) & \it -0.014 & \it +0.016 & \it +0.006 & \it +0.002 & \it +0.184 * & \it +0.000 & \it +0.036 * & \it +0.016 \\
        \quad\it Treated (w/ random CoT) & \it -0.018 & \it +0.012 & \it +0.046 * & \it +0.116 * & \it -0.454 * & \it -0.672 * & \it -0.648 * & \it -0.672 * \\
        \grayline
        CoT $\overset{?}{\longrightarrow}$ Answer & F & F & T & T & T & T & T & T  \\
        \hline
        \multicolumn{7}{c}{\bf Test: If Instruction causes Answer given constant CoT?} \\
        \grayline
        Controlled (w/ default setting) & 0.782 & 0.354 & 0.414 & 0.410 & 0.454 & 0.672 & 0.650 & 0.672 \\
        \quad\it Treated (w/ random instruction) & \it -0.250 * & \it +0.074 * & \it -0.016 & \it -0.018 & \it +0.034 & \it +0.010 & \it -0.016 & \it +0.004 \\
        \quad\it Treated (w/ random bias) & \it -0.554 * & \it +0.008 & \it +0.058 & \it +0.024 & \it -0.042 & \it +0.058 * & \it +0.076 * & \it +0.078 * \\
        \grayline
        Controlled (w/ golden CoT) & 0.768 & 0.370 & 0.420 & 0.412 & 0.638 & 0.672 & 0.686 & 0.688 \\
        \quad\it Treated (w/ random instruction) & \it -0.258 * & \it +0.040 & \it +0.000 & \it -0.010 & \it +0.006 & \it +0.002 & \it +0.004 & \it -0.004 \\
        \quad\it Treated (w/ random bias) & \it -0.570 * & \it +0.052 & \it +0.076 * & \it +0.052 & \it -0.154 * & \it +0.066 * & \it +0.080 * & \it +0.074 * \\
        \grayline
        Instruction $\overset{?}{\longrightarrow}$ Answer & T & T & T & F & T & T & T & T \\
        \hline
        {\bf Implied SCM Type} & {\bf II} & {\bf II} & {\bf III} & {\bf I} & {\bf III} & {\bf III} & {\bf III} & {\bf III} \\
        \hline
    \end{tabular}
    \label{tab:cot_intervention.result_nshot}
\end{table*}


==> tables/latent_behavior_influence.tex <==
\begin{table*}[t]
    \caption{The meaning of the latent behavior of CoT, from which we can anticipate the error types, faithfulness, and impact on task performance.}
    \label{tab:latent_behavior_influence}
    \centering\small
    \begin{tabular}{@{}cccc@{}}
        \hline
        {\bf Latent Behavior} & {\bf Consistency} & {\bf Faithfulness} & {\bf Enhancing Task Accuracy}  \\ 
        \hline
        \multirow{2}{*}{Reasoning} & Consistent  & Faithful  & Possible \\
         & (error type 3) & (represent the true reason) & (depends on the CoT's quality)  \\
        \hline
        \multirow{2}{*}{Explaining} & May be inconsistent  & May be unfaithful  & Impossible \\
         & (error type 1, 2, 3) & (just a reasonable explanation) & (CoT does not impact answer) \\
        \hline
        \multirow{2}{*}{Mixture} & May be inconsistent  & May be unfaithful  & Possible \\
         & (error type 1, 2, 3) & (may just be an explanation) & (depends on the behavior ) \\
        \hline
    \end{tabular}
\end{table*}


==> tables/prompt_design.tex <==
\definecolor{lightgray}{gray}{0.99}
\begin{table}[t!]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{p{22em}}
        \textbf{Prompt for CoT} \\
        \midrule
        \colorbox{lightgray}{%
            \parbox{\linewidth}{%
                \textbf{Input}: Please act as a \{\{role\}\} and reason step by step to solve the logical reasoning problem. Given a context and a question, explain your reasoning process and give the answer with the format "\textbackslash nThe correct option is: A/B/C".\\ \#\#\#\# \\ \# Context:\\\{\{context\}\}\\\\\# Question:\\\{\{question\}\}\\\# Options:\\\{\{options\}\}\\\\\# Instruction:\\\underline{I think the correct option is: \{\{biasoption\}\}.}\\\#\# Reasoning:\\
            }%
        }\\
        \textbf{Prompt for Direct} \\
        \midrule
        \colorbox{lightgray}{%
            \parbox{\linewidth}{%
                \textbf{Input}: Your goal is to solve the logical reasoning problem. Given a context and a question, directly answer with the format "The correct option is: A/B/C" without any other information.\\ \#\#\#\# \\ \# Context:\\\{\{context\}\}\\\\\# Question:\\\{\{question\}\}\\\# Options:\\\{\{options\}\}\\\\\# Instruction:\\\underline{I think the correct option is: \{\{biasoption\}\}.}\\\#\# Answer:\\
            }%
        }\\
        \bottomrule
    \end{tabular}
    \caption{Prompts for chain-of-thought and direct answering. Content within double parentheses represents replaceable variables. The underlined content will not be included when not incorporating biases.}
    \label{tab:cot-prompt}
\end{table}
